Embedding-based Zero-shot Retrieval through Query Generation

Passage retrieval addresses the problem of locating relevant passages, usually from a large corpus, given a query. In practice, lexical term-matching algorithms like BM25 are popular choices for retrieval owing to their efficiency. However, term-based matching algorithms often miss relevant passages that have no lexical overlap with the query and cannot be finetuned to downstream datasets. In this work, we consider the embedding-based two-tower architecture as our neural retrieval model. Since labeled data can be scarce and because neural retrieval models require vast amounts of data to train, we propose a novel method for generating synthetic training data for retrieval. Our system produces remarkable results, significantly outperforming BM25 on 5 out of 6 datasets tested, by an average of 2.45 points for Recall@1. In some cases, our model trained on synthetic data can even outperform the same model trained on real data

==> tables/ablation_msmarco.tex <==
\begin{table}[h!]
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize
\begin{tabu}{@{}lcccc@{}}
\toprule
\multirow{2}{*}{\textbf{Pooling}} & Dataset & \multicolumn{3}{c}{\textsc{Natural Questions}}  \\
& R@1 & R@10 & R@100 \\
\midrule
BM-25 & 0.307 & 0.638 & 0.82 \\
\midrule
Siamese CLS-512 & Text & \textbf{-} & \textbf{-} & \textbf{-} \\
Siamese mean-512 & Text & - & - & - \\
Siamese max-512 & 0.Text & - & - & - \\
\midrule
Two-Tower CLS-512 & Text & \textbf{-} & \textbf{-} & \textbf{-} \\
Two-Tower mean-512 & Text & - & - & - \\
Two-Tower max-512 & Text & - & - & - \\
\bottomrule
\end{tabu}
\end{minipage}
\caption{Ablation study comparing against a model trained on \textsc{MSMARCO} ground truth data.}
\label{table:ablation_pooling}
\end{table}

==> tables/ablation_pooling.tex <==
\begin{table}[h!]
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize
\begin{tabu}{@{}lccc@{}}
\toprule
\multirow{2}{*}{\textbf{Pooling}} & \multicolumn{3}{c}{\textsc{Natural Questions}}  \\
& R@1 & R@10 & R@100 \\
\midrule
BM25 & 30.7 & 63.8 & 82.0 \\
\midrule
Siamese \texttt{CLS}-512 & \textbf{41.0} & \textbf{81.1} & \textbf{95.1} \\
Siamese \texttt{mean}-512 & 38.5 & 80.7 & 95.1 \\
Siamese \texttt{max}-512 & 39.4 & 78.5 & 93.9 \\
\midrule
Two-Tower \texttt{CLS}-512 & \textbf{34.9} & \textbf{76.3} & \textbf{93.5} \\
Two-Tower \texttt{mean}-512 & 32.5 & 75.2 & 89.8 \\
Two-Tower \texttt{max}-512 & 30.5 & 71.1 & 91.8 \\
\bottomrule
\end{tabu}
\end{minipage}
\caption{Ablation study over various types of pooling over the final layer BERT representations. 512 is the embedding size. Numbers are in percent (\%).}
\label{table:ablation_pooling}
\end{table}
